Real Negatives Matter: Continuous Training with Real Negatives for Delayed Feedback Modeling

One of the difficulties of conversion rate (CVR) prediction is that the conversions can delay and take place long after the clicks. The delayed feedback poses a challenge: fresh data are beneficial to continuous training but may not have complete label information at the time they are ingested into the training pipeline. To balance model freshness and label certainty, previous methods set a short waiting window or even do not wait for the conversion signal. If conversion happens outside the waiting window, this sample will be duplicated and ingested into the training pipeline with a positive label. However, these methods have some issues. First, they assume the observed feature distribution remains the same as the actual distribution. But this assumption does not hold due to the ingestion of duplicated samples. Second, the certainty of the conversion action only comes from the positives. But the positives are scarce as conversions are sparse in commercial systems. These issues induce bias during the modeling of delayed feedback. In this paper, we propose DElayed FEedback modeling with Real negatives (DEFER) method to address these issues. The proposed method ingests real negative samples into the training pipeline. The ingestion of real negatives ensures the observed feature distribution is equivalent to the actual distribution, thus reducing the bias. The ingestion of real negatives also brings more certainty information of the conversion. To correct the distribution shift, DEFER employs importance sampling to weigh the loss function. Experimental results on industrial datasets validate the superiority of DEFER. DEFER have been deployed in the display advertising system of Alibaba, obtaining over 6.0% improvement on CVR in several scenarios. The code and data in this paper are now open-sourced {https://github.com/gusuperstar/defer.git}.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> deploy.tex <==
\section{Online Serving}
\subsection{Challenges}
\subsection{Solution}
\begin{itemize}
	\item sequence cutoff and feature dim reduction
	\item less orders
	\item kernel optimazation
\end{itemize}
\subsection{Results}

==> experiments.tex <==
\begin{table*}[t]
	\caption{The example percentage of each domain.}
	\label{table:sample_percentage}
	\resizebox{\textwidth}{!}{\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
	\toprule
	         &1 & 2& 3& 4& 5& 6& 7& 8& 9& 10& 11& 12& 13& 14& 15& 16& 17& 18& 19\\
	\midrule
	Percentage &0.99\% & 1.61\% &3.40\% &3.85\% &2.79\% &0.56\% &4.27\% &16.76\% &10.00\% &12.16\% &0.76\% &1.31\% &3.34\% &28.76\% &1.17\% &0.46\% &1.05\% &0.91\% &5.85\%   \\
	\bottomrule
	\end{tabular}}
\end{table*}
\section{Experiments}

We evaluate the efficacy of STAR in this section. We begin by introducing the setup including the used production dataset, compared method and implementation details in Sec.~\ref{sec:setting}.  The results and discussion are elaborated in Sec.~\ref{sec:res}. We also perform in-depth ablation studies in Sec.~\ref{sec:ablation}. Experimental results on production environment are shown in Sec.~\ref{sec:industrial}.

\subsection{Experimental Settings}\label{sec:setting}



\textbf{Dataset.} We use Alibaba production data regarding user click behavior on 19 business domains to perform the offline evaluation.  The training data is collected from traffic logs of the online display advertising system of Alibaba. Data of one day from 19 business domains are used for training and the data of the following day is used for testing. The training dataset consists of  billions of examples. \ref{table:sample_percentage} shows the example percentage of each domain in the training set.


\textbf{Compared models.}
To verify the effectiveness of the proposed approach, we compare STAR with the following models:
\begin{itemize}
    \item \textbf{Base}. We refer to Base as the model composed of embedding layer, pooling \& concatenation layer, batch normalization and a 7-layer fully-connected networks. Specifically, the pooling \& concatenation layer is based on DIEN~\cite{zhou2019dien}, which extracts user interest after the embedding layer. After the extraction. We mix all samples from different domains and train the base model.
    \item \textbf{Shared Bottom}. The Shared Bottom model is a multi-task model that shares the parameters of bottom layers. In our implementation, we let the Shared Bottom share the embedding layer and interest extraction layer. Each domain will also have a specific 7-layer fully-connected network that is not shared.
    \item \textbf{MMoE}. MMoE~\cite{MaZYCHC2018MMOE} implicitly models task relationship for multi-task learning, where different tasks may have different label spaces. Here we adapt MMoE for multi-domain CTR prediction, where each  fully-connected network is treated as an expert. The number of expert is equal to the number of domains. Besides, MMoE also learns   gating networks per domain that takes the input features and outputs softmax gates assembling the experts with different weights. 
\end{itemize}
To give a fair comparison, all compared methods and the STAR model are trained with the proposed auxiliary network in Sec.~\ref{sec:res}. The ablation study about the auxiliary network is performed in Sec.~\ref{sec:ablation}.

\textbf{Implementation details.} 
All models are trained with Adam~\cite{KingmaB2014Adam}, the learning rate is set to 0.001 and the batch size is 2000. We minimize the cross-entropy loss for samples from all domains to train the model.

\textbf{Metrics.} 
Area under the ROC curve (AUC) is the common metric used to evaluate the performance of CTR prediction. An variation of user weighted AUC~\cite{zhou2018din}  measures the goodness of intra-user order by averaging AUC over users and is shown to be more relevant to online performance in display advertising system. It is calculated as follows:
\begin{equation}
    \textrm{AUC} = \frac{\sum_i^n \# \textrm{impression}_i \times \textrm{AUC}_i}{\sum_i^n \# \textrm{impression}_i},
\end{equation}
where $n$ is the number of users, $\textrm{impression}_i$ and $\textrm{AUC}_i$ are the number of impressions and AUC of the $i$-th user, respectively. 
We use this weighted AUC as the evaluation metric and still refer it as AUC for simplicity. Concretely, we use the AUC of each domain and overall AUC (mixing samples from all domains to calculate the overall AUC) as the metrics.  

\subsection{Results}\label{sec:res}
We evaluate all approaches on Alibaba production dataset. To give a fair comparison, all compared methods and the STAR model are trained with the proposed auxiliary network. The result is shown in  Table~\ref{table:offline_result}. As illustrated in Table~\ref{table:offline_result}, 
the Shared Bottom model, MMoE and STAR all achieve better overall performance than Base model. This demonstrate the importance of exploiting domain relationship and capturing domain distinction to enhance the prediction performance. The consistent improvement validates the efficacy of STAR. 

Although the Shared Bottom and MMoE achieve better overall performance than the Base model, note that in some domains, the performance of Shared Bottom and MMoE is worse than the Base model, e.g., domain \# 5 and \#16.
In contrast, the proposed STAR model exhibits superior performance across all domains comparing with the Base model. Besides, STAR also achieves consistent improvement than the Shared Bottom, which demonstrates the importance of information sharing on top layers for multi-domain learning where all domains shares the same label space. STAR also outperforms MMoE, which shows the superiority of explicitly model domain relationship compared with implicitly implicitly model domain relationship by the gate networks. 


% \begin{table}[t]
% 	\caption{Results of different approaches on offline production dataset.}
% 	\label{table:offline_result}
% 	\begin{tabular}{c|c|c|c|c}
% 	\toprule
% 	        & Base & Multi-Head & MMoE & STAR \\
% 	\midrule
% 	\#1           &0.6134&0.6103 &0.6135                     & 0.6306       \\
% 	\#2           &0.6321&0.6258 &0.6323 & 0.6417        \\
% 	\#3           &0.6281&0.6238 &0.6282 & 0.6372        \\
% 	\#4           &0.6326&0.6301 &0.6328 & 0.6451        \\
% 	\#5           &0.6308&0.6230 &0.6302 & 0.6388        \\
% 	\#6           &0.6378&0.6342 &0.6359 & 0.6494        \\
% 	\#7           &0.6305&0.6278 &0.6305 & 0.6410        \\
% 	\#8           &0.6297&0.6278 &0.6295 & 0.6411        \\
% 	\#9           &0.6264&0.6237 &0.6262 & 0.6368        \\
% 	\#10           &0.6392&0.6348 &0.6359 & 0.6577 \\
% 	\#11          &0.6469 &0.6404 &0.6434 & 0.6719        \\
% 	\#12           &0.6506&0.6464 &0.6461& 0.6676        \\
% 	\#13           &0.6558&0.6527 &0.6530& 0.6739        \\
% 	\#14           &0.6362&0.6360 &0.6370& 0.6486        \\
% 	\#15           &0.6043&0.5577 &0.5918& 0.5851        \\
% 	\#16           &0.6745&0.6769 &0.6696 & 0.7021        \\
% 	\#17           &0.6638&0.6684 &0.6491& 0.6901        \\
% 	\#18           &0.6524&0.6581 &0.6476 & 0.6715        \\
% 	\#19           &0.6493&0.6480 &0.6352 & 0.6754        \\
% 	\#20           &0.6330&0.6304 &0.6297 & 0.6476        \\
% 	\midrule
% 	Average AUC            & 0.000 &0 & &  0.000       \\
% 	Overall AUC & 0.6364 &0.6343 & 0.6345& 0.6506        \\
% 	\bottomrule
% 	\end{tabular}
% \end{table}

\begin{table}[t]
	\caption{Results of different approaches on offline Alibaba production dataset.}
	\label{table:offline_result}
	\begin{tabular}{c|c|c|c|c}
	\toprule
	        & Base & Shared Bottom & MMoE  & STAR \\
	\midrule
	\#1
	&0.6134&0.6186&0.6143& \textbf{0.6306 }      \\
	\#2
	&0.6321&0.6320&0.6355 & \textbf{0.6417}        \\
	\#3           &0.6281&0.6293&0.6311 & \textbf{0.6372}        \\
	\#4 &0.6326&0.6361&0.6373 & \textbf{0.6451}        \\
	\#5
	&0.6308&0.6292&0.6336& \textbf{0.6388}        \\
	\#6
	&0.6378&0.6383 &0.6412& \textbf{0.6494}        \\
	\#7
	&0.6305&0.6329 &0.6340& \textbf{0.6410}        \\
	\#8
	&0.6297&0.6278 &0.6330&\textbf{0.6411}        \\
	\#9
	&0.6264&0.6283&0.6292& \textbf{0.6368}        \\
	\#10
	&0.6392&0.6434 &0.6431& \textbf{0.6577} \\
	\#11
	&0.6469 &0.6529&0.6508& \textbf{0.6719}        \\
	\#12
	&0.6506&0.6575
	& 0.6518&\textbf{0.6676}        \\
	\#13
	&0.6558&0.6612 &0.6603& \textbf{0.6739}        \\
	\#14
	&0.6362&0.6405 &0.6412& \textbf{0.6486}        \\
% 	\#15
% 	&0.6043&0.5739 &0.6207& 0.5851        \\
	\#15
	&0.6745&0.6888 &0.6787& \textbf{0.7021}        \\
	\#16&0.6638&0.6627 &0.6634& \textbf{0.6901}        \\
	\#17&0.6524&0.6658 &0.6519& \textbf{0.6715}        \\
	\#18 &0.6493&0.6480&0.6500 & \textbf{0.6754}        \\
	\#19 &0.6330&0.6375&0.6374 & \textbf{0.6476}        \\
	\midrule
% 	Average AUC & 0.000 &0  &  0.000 &0.000      \\
	Overall AUC & 0.6364 & 0.6398 &0.6403 & \textbf{0.6506}        \\
	\bottomrule
	\end{tabular}
\end{table}

\subsection{Ablation Study}\label{sec:ablation}

To investigate the effect of each component, we conduct several ablation studies.



































































































\subsubsection{STAR FCN and PN} 

\begin{table}[t]
	\caption{Ablation study of partitioned normalization (PN) and star topology fully-connected neural networks (STAR FCN). All models are trained with the proposed auxiliary network.}
	\label{table:ablation_shadow}
	\resizebox{\columnwidth}{!}{\begin{tabular}{c|c|c|c|c}
	\toprule
	  &    Base (BN)  & Base (PN) & STAR FCN (BN) & STAR FCN (PN) \\
	\midrule
% 	Average AUC           & 0.000 &0.000&0.000&0.000\\
	Overall AUC & 0.6364 &0.6485 & 0.6415 &  \textbf{0.6506}    \\
	\bottomrule
	\end{tabular}}
\end{table}
We analyze the influence of different components of STAR. Concretely, the separate effects of star topology fully-connected neural networks (STAR FCN)  and partitioned normalization (PN) are investigated. We compare the Base model trained with BN, Base model trained with PN, STAR FCN with BN and the STAR model (STAR FCN + PN). The result is reported  in Table~\ref{table:ablation_shadow}. 
We observe that using only shadow brings xx\% improvement and using only SSLT brings xx\% improvement. Bring them together improves XX\% compared with the Base model. The result validates the effect of both STAR FCN and PN.

\subsubsection{Normalization}
Normalization methods are very effective component in deep learning, which have been shown by many practices to ease optimization and enable very deep networks to converge. We analyze the effect of different normalization methods including Batch Normalization (BN)~\cite{PiBZZG19MIMN}, Layer Normalization (LN)~\cite{BaKH2016LN} and the proposed Partitioned Normalization (PN) on multi-domain CTR prediction. BN accumulates global statistics and learns global parameters for samples from all domains. LN is a representative instance-based normalization method, which operates along the channel dimension and avoid mixing statistics for samples from different domains. 

The result is shown in Table~\ref{table:ablation_normalization}.
Our first observation is that both LN and PN outperforms BN. This observation validates that data from different domains have distinct distribution. Thus  global normalization methods obscure domain differences. which will not perform well on multi-domain CTR prediction.
We find PN outperforms LN, this validates that  privatizing normalization for samples from different domains outperforms operating normalization  only for each sample since PN leads to more accurate moments.

\begin{table}[t]
	\caption{Ablation study of normalization methods for multi-domain CTR prediction. STAR FCN is trained BN, LN and PN respectively.}
	\label{table:ablation_shadow}
	\resizebox{\columnwidth}{!}{\begin{tabular}{c|c|c|c}
	\toprule
	  &STAR FCN (BN) &    STAR FCN (LN) & STAR FCN (PN) \\
	\midrule
% 	Average AUC           & 0.000 &0.000&0.000&0.000\\
	Overall AUC &0.6415 & 0.6463 &  \textbf{0.6506}    \\
	\bottomrule
	\end{tabular}}
\end{table}

\subsubsection{Auxiliary network} 
We conduct experiment to assess the effect of auxiliary network for different models. Base model, Shared Bottom model, MMoE and STAR are trained with and without auxiliary network. The result is illustrated in Figure~\ref{fig:ablation_auxiliary}. We observe that auxiliary network improves base model, Shared Bottom model,  MMoE and STAR consistently. The result  validates the importance of making full utilization of domain features and capturing the domain distinction.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figure/eval_aux.pdf}
    \caption{The performance of different methods trained without and with auxiliary network.}
    \label{fig:ablation_auxiliary}
\end{figure}

% \textbf{Normalization} 
% \begin{table}[t]
% 	\caption{The effect of different  normalization methods.}
% 	\label{table:ablation_normalization}
% 	\begin{tabular}{c|c|c|c|c}
% 	\toprule
% 	  &    BN   & LN & SBN  \\
% 	\midrule
% 	Average AUC           & 0.000 &0.000&0.000\\
% 	Overall AUC  &0.000&0.000 &0.000      \\
% 	\bottomrule
% 	\end{tabular}
% \end{table}


\subsection{Production}\label{sec:industrial}
\textbf{Online serving and challenges.} 
One of the challenges in industrial recommender is that the distribution of features and click through rate (CTR) exhibits large shifts over time. 
To capture the dynamic change of data in real time, it is important to use the real-time examples to update the CTR models continuously to prevent them from becoming stale. 
% The common way to organize input data for CTR prediction is to abstract data in the domain-level. The domain-level abstraction treats each domain independently and organizes domain-specific data for each domain. To combine data from multiple domains, it needs large development cost. If we want to add new domains and combine data from different sources, it need re-develop a new dataflow to construct the input data. The re-development is both inefficient and time-consuming, which is due to the lack of flexibility and information reuse.To address this issue, we optimize the online data flow where basic data unit flow as the minimal unit and takes it as input dataflow. Different input dataflows can be split and assembled flexibly for different tasks. This implementation enables efficient algorithm iteration on online data from multiple business domains.
However, for multi-domain CTR prediction, the real-time example percentage of each domain changes over time. For example, some business domains have  traffic spike on morning while  some business domains have  traffic spike on evening. If we mix real-time samples from all domains for each mini-batch according to chronological order, the changes of data percentage over time will cause the instability of model learning. To address this issue, we redesign the data pipeline, where each batch only contain examples from a single business domain. Besides, we maintain a buffer that store history samples. Samples are shuffled and then  feed to the model to avoid the sudden change of example percentage. After that, this mini-batch of samples are removed from the buffer. We empirically found this training manner is more stable than the traditional way of online update. 


The systematical optimization makes STAR capable of serving main traffic from multiple business domains stably. Table~\ref{tab:production} shows the improvement of STAR on the display advertising system of Alibaba. We compute the overall improvements on all domains. The introduction of STAR brings +8.0\% overall CTR lift and +6.0\% overall RPM (Revenue Per Mille) lift in our online A / B test compared with the Base model. 
\begin{table}[t]
	\caption{CTR and RPM gains in online display advertising system of Alibaba.}
	\label{tab:production}
	\begin{tabular}{l|l|l}
	\toprule
	         & CTR & RPM \\
	\midrule
	Overall   & +8.0\%  & +6.0\% \\
	\bottomrule
	\end{tabular}
\end{table}





==> method.tex <==
\section{The Proposed Approach}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figure/STAR.pdf}
    \caption{Overview of Star Topology Adaptive Recommender (STAR) for multi-domain CTR prediction. STAR consists of three main components: (1) the partitioned normalization (PN) which privatizes normalization for examples from different domains, (2) the star topology full-connected neural network (Star Topology FCN) which consists of shared centered FCN and multiple independent FCNs. The final model of each domain is obtained by element-wise product of weights in each layer.  (3) the auxiliary network which treats the domain indicator directly as the input feature to capture the domain distinction.}
    \label{fig:shadow}
\end{figure*}
In this section, we first give a brief introduction about the background of multi-domain CTR prediction. Next are the architecture overview of our  method, star topology adaptive recommender for multi-domain CTR prediction. 
Then we introduce STAR in detail, including the proposed star topology network, partitioned normalization and auxiliary network. 
% Finally are our practical lessons learned in deploying STAR to production.
\subsection{Multi-Domain CTR Prediction}
In sequential recommender systems, the model takes input as the user historical behavior, user profile feature, target item feature and other features like  context feature.
The CTR $\hat{y}$ of an user $u$ clicking on an item $m$ is calculated via: 
\begin{equation*}
    \hat{y} = \mathrm{f}(E(u_1),\dots,E(u_i);E(m_1),\dots,E(m_j);E(c_1),\dots,E(c_k)),
\end{equation*}
where $\{u_1,\dots,u_i\}$ is the set of user features including user historical behavior and user profile feature. $\{m_1,\dots,m_i\}$ is the set of target item feature and $\{c_1,\dots,c_i\}$ is the set of other features. The $E(\cdot)\in \mathbb{R}^d$ means the embedding layer which maps the sparse IDs into learnable dense vector. 

After mapping the raw features to low-dimensional embeddings, the common practice is to aggregate these embeddings to obtain fixed-length vectors. Different kinds of aggregation methods like~\cite{zhou2018din,zhou2019dien}  are proposed to aggregate these embeddings to extract user interest and get the fixed-length representation. The obtained representation are then fed into the following deep neural network, e.g., a multi-layer fully-connected network, to get the final CTR prediction.

Traditional CTR models~\cite{guo2017deepfm,lian2018xdeepfm,cheng2016wide,zhou2018din,zhou2019dien} are usually trained on data from a single business domain. However, real-world recommender often have to  deal with multiple business domains. To enhance user satisfaction and promote advertising revenue, it is necessary to give accurate prediction for request from all domains. Concretely, the recommender needs to  make CTR prediction for $M$ domains $D_1, D_2, \dots, D_M$ simultaneously. The model takes input as $(\x, y, p)$, where $\x$ is the common feature used by multiple business domains like user historical behavior and user profile feature, target item feature as mentioned above. $y \in {0, 1}$ is the clicked label and $p \in \{1, 2, \dots, M\}$ is the domain indicator that indicates which domain this sample is collected. Note that each instance $\x$ is drawn from the domain-specific distribution $D_p$ and the distribution varies for different domains. 
The goal of multi-domain CTR prediction is to construct a single CTR model that can give accurate CTR prediction to serve all domains at low resource consumption and human cost.


\subsection{Architecture Overview}

As mentioned above, ignoring domain indicator $p$ and learning a single  shared CTR model neglect the domain differences. This leads to inferior model performance. On the other hand, training separate models for each domain performs much worse since splitting the domains provides much less data for each model and makes it hard to fit complicated  deep neural networks. Besides, due to the resource consumption and human cost, it is infeasible to maintain each domain a separate model in production. 

To this end, we propose Star Topology Adaptive Recommender (STAR)  for multi-domain CTR prediction to better utilize the similarity among different domains while capture the domain distinction.  
As shown in Figure~\ref{fig:shadow}, STAR consists of three main components: (1) the \textbf{partitioned normalization} (PN) which  privatizes normalization for examples from different domains, (2) the \textbf{star topology full-connected neural network} (Star Topology FCN) which consists of shared centered parameters and multiple set of domain-specific parameters. The final model of each domain is obtained by combining  the shared centered parameters and domain-specific parameters.   (3) the \textbf{auxiliary network} which treat the domain indicator directly as the input feature and learns its semantic embeddings to capture the domain distinction.

Concretely, given a mini-batch of $B$ instances $$(\x_1, p), (\x_2, p), \dots, (\x_B, p)$$ from the $p$-th domain, STAR first embeds these input features as low-dimensional vectors by an embedding layer. In industrial recommender, the model is often trained with billions of features~\cite{Jiang2019XDL}.  Due to the large amount of features,  the parameters of embedding  are usually much more than other parts of model, which make it difficult for different domain to learn domain-specific embeddings with limited data.
Thus, in the proposed STAR model, we let all business domains share the same embedding layer, i.e., same ID features in different domains will share the same embedding. 
 Let the embedding layers to be shared across multiple domains can significantly reduce the computational and memory cost.
For example, for models used in our daily tasks, the embeddings parameters is 10,000 times more than  the parameters of multi-layer fully connected networks~\cite{Jiang2019XDL}. Thus we let the embedding layers to be shared across multiple domains considering the computational and memory cost.

The embeddings are then pooled and concatenated to obtain $B$ fixed-length representations. After that, the $B$ extracted representations are processed by the proposed partitioned normalization (PN) layer that privatizes normalization statistics for different domains. During training, PN employs the batch statistics just as the batch normalization~\cite{IoffeS2015BN}, but employs independent  mean and variance for different domains during testing.
The normalized vectors are then fed as input to the proposed star topology multi-layer fully-connected neural network (FCN) to get the output. The star topology FCN consist of shared centered FCN and multiple set of domain-specific FCNs. The final model of each domain is obtained by combining  the shared centered FCN and domain-specific FCN, which is implemented by the element-wise product of between weights in each layer. The purpose of the centered parameters is to learn general behaviors among all domains, in which the common knowledge are learned and transferred among all domains.  The domain-specific parameters capture specific behaviors in different domains to facilitate more refined CTR prediction. The star topology facilitates effective information transformation across multiple domains to learn domain commonalities and distinction.

In multi-domain CTR prediction, features that depict the domain information is of importance. In STAR model, the auxiliary network treats the domain indicator as the ID feature. The domain indicator is first mapped into   embedding and then fed with other features depicting the domain to the auxiliary network.  The output of the auxiliary network is added with the output of the star topology FCN to get the final prediction.
We make the auxiliary network much simpler than the star topology FCN to make the model capture the domain distinction in a direct and easy manner.

In what follows we will describe these components in detail.





\subsection{Partitioned Normalization}
% In industrial recommender, the model is often trained with billions of features~\cite{Jiang2019XDL}. The common operation is encode each feature into an one-hot vector then transformed into low-dimensional dense features by embedding
% layer. Due to the large amount of features,  the parameters of embeddings  are usually much more than other parts of model like FCN, which make it difficult for different domain to learn domain-specific embeddings with limited data.
% Thus, in the proposed STAR model, we let all business domains share the same embedding layer, i.e., same ID features in different domains will share the same embedding. 
% A simple methods to obtain the sample representation is concatenating the embeddings of each feature. However, in practice, it's important to capture user interest in user behaviors. Thus we adopt the attention mechanism with GRU to model dynamic evolution of user interest for feature aggregation as DIEN~\cite{zhou2019dien}. The GRU and attention parameters are also shared by all domains. 
As mentioned above, the raw features are first transformed into low-dimensional embeddings and then pooled and aggregated to get the intermediate representation. Denote the the intermediate representation of a instance as $\z$, to train deep networks fast and stably, a standard practice is applying normalization layer to the intermediate representation $\z$. 
Among all normalization methods, batch normalization (BN)~\cite{IoffeS2015BN} is a representative method that is proved to be crucial to the successful training of very deep neural networks~\cite{IoffeS2015BN,RadfordMC2015UnsupervisedGAN}. 
% Batch normalization (BN) is XXX are mean and variance of current mini-batch during training. During testing, moving averaged statistics of means and variances across all training images are used instead. 
BN use a global normalization for all examples, which accumulates  normalization moments and learns shared parameters across all samples. Concretely, the normalization of BN in training is given as  
\begin{equation}
    \z^{\prime} = \gamma\frac{\z - \mu}{\sqrt{\sigma^2+\epsilon}} + \beta,
\end{equation}
where $\z^{\prime}$ is the output, $\gamma, \beta$ are the learnable scale and bias parameters, $\mu, \sigma^2$ are mean and variances of current mini-batch.
During testing, moving averaged statistics of mean $E$ and variance $Var$ across all samples are used instead
\begin{equation}
    \z^{\prime} = \gamma\frac{\z - E}{\sqrt{Var+\epsilon}} + \beta.
\end{equation}
In other words, traditional methods assume all samples are i.i.d. and use the shared statistics across all training samples.

However, in multi-domain CTR prediction, samples are only assumed to be locally i.i.d. within in a specific domain. Thus, data from different domains have different normalization moments. Sharing global moments and parameters of BN layer during testing will obscure domain differences and lead to degraded  model performance. To capture the unique data characteristic of each domain, we propose partitioned normalization (PN) which privatizes normalization statistics and parameters for different domains. Concretely, during training, suppose the current  mini-batch is sampled from the $p$-th domain, we compute the mean and variances of current mini-batch and normalize the feature as:
\begin{equation}
    z^{\prime} = (\gamma*\gamma_p)\frac{z - \mu}{\sqrt{\sigma^2+\epsilon}} + (\beta+\beta_p),
\end{equation}
where $\gamma, \beta$ are the global scale and bias and $\gamma_p, \beta_p$ are the domain-specific scale and bias parameters. For each mini-batch, it receives the final scale  by element-wise multiplying the shared $\gamma$ with the domain-specific $\gamma_p$, i.e., PN adaptively scales the representation according to the domain indicator. Similarly, the bias of PN is also adaptive  according to the domain indicator, which is implemented by the sum of global bias $\beta$ and domain specific bias $\beta_p$.
Note that compared with BN, PN also uses the moments of the current mini-batch, but PN introduces domain-specific scale and bias  $\gamma_p, \beta_p$ to capture the domain distinction. 

Besides the modification of the scale and bias, PN also let different domains to accumulate its domain-specific moving average of mean $E_p$ and variance $Var_p$. 
During testing, PN transforms  instance $\z$ from the $p$-th domain as:
\begin{equation}
    \begin{aligned}
        \z^{\prime} = (\gamma*\gamma_p)\frac{\z - E_p}{\sqrt{Var_p+\epsilon}} + (\beta+\beta_p).
    \end{aligned}
    \label{eq:pn}
\end{equation}
% μi =αE[xi]+(1−α)mx
% σi2 =(αE[x2i]+(1−α)mx2)−μ2i
From Equation~\ref{eq:pn}, we can see that PN use the domain-specific mean $E_p$ and variance $Var_p$ to normalize the intermediate representation $\z$. Thus PN adaptively alters the intermediate representation according to the domain indicator to capture the distinctive characteristics. 


% To discover important distinctions between features in different domains, we perform a domain-specific element-wise linear transformation to the representation $\z$, that is,
% \begin{equation}
%     H(\z) = \z \otimes \bm \beta_p + \gamma_p
% \end{equation}
% where $f_p$ has the same dimension with $\z$ and $\otimes$ is the element-wise product. 

\subsection{Star Topology FCN}
After the PN layer, the representation $\z^{\prime}$ is fed as input to the following star topology multi-layer fully-connected neural network (star topology FCN).
As depicted in Figure~\ref{fig:shadow}, the proposed star topology FCN consists of a shared centered FCN and independent FCNs per domain, thus the total number of FCN is $M+1$. The final model of $p$-th domain is obtained  by combining the shared centered parameters and domain-specific parameters, in which the centered parameters learn general behaviors among all domains and the domain-specific parameters capture specific behaviors in different domains to facilitate more refined CTR prediction. 

% Compared with using a shared FCN obscures domain distinctions, we introduces star topology FCNs  to capture the domain differentce while learning the commonality. 

Specifically, for the shared FCN, let $W$ be the weights  and $b$ be the bias in a  neural network layer respectively. For the independent FCN of the $p$-th domain, let $W_p$ be the weights  and $b_p$ be the bias in the corresponding  layer.
Denote the input dimension as $c$ and the output dimension as $d$, i.e, $W, W_p\in \mathbb{R}^{c\times d}, b, b_p\in \mathbb{R}^d$. 
The final weights $W^{\star}_i$ and bias $b^{\star}_i$ for the $p$-th domain is obtained by:
\begin{equation}
    W^{\star}_p =  W_p \otimes W, b^{\star}_p = b_p + b, 
    \label{eq:shadow}
\end{equation}
where  $\otimes$ denotes the element-wise multiplication. Let $in_p \in \mathbb{R}^{c\times 1}$ denote the  input of this neural network layer from the $p$-th domain, the final output $out_p \in \mathbb{R}^{d} \times 1$ is given by:
\begin{equation}
    out_p = \phi((W^{\star}_p)^\top in_p + b^{\star}_p),
\end{equation}
where $\phi$ denotes the activation function of this layer.  The combination of shared parameters of domain-specific parameters is applied in all layers. 

Note that we implement the combination strategy of the shared centered FCN and domain-specific FCN by element-wise product of between weights and addition of bias in each layer, other strategy can also be investigated for better performance. As shown in~\ref{eq:shadow}, the domain-specific parameters $W_p$ and $b_p$  selectively modulating the shared weights $W$ and bias $b$ based on the characteristic of the current domain. This helps capturing the domain differences for more refined CTR prediction while learning the domain commonality through the shared centered parameters. 
As mentioned above, most of the parameters in industrial recommender is taken account by embedding layer, the added $M$ FCNs is negligible to the total amount of parameters.
By adaptively changing its behaviors for different domains, STAR uses one model to effectively serve all business domains in a  parameter efficient and memory friendly manner.
% The introduction of element-wise transformation and Shadow of FCN improve the ability to capture the domain differences. The element-wise transformation empower the model to manipulate the immediate representation by scaling each feature. Shadow of FCN empower the model to 

\subsection{Auxiliary Network}
In the traditional way of CTR modeling, all features are treated equally and fed to the complicated model. In multi-domain CTR prediction, however, it may be hard for the model to automatically learning the domain distinction. We argue that a good multi-domain CTR model should have the following characteristic: (1) have informative features regarding the domain characteristic (2) make these feature easily and directly influence the final CTR prediction. The intuition behind is that features that depicts the information of domains are of importance, since it can reduce the difficulty for the model to capture the distinction among domains.

To this end, we propose an auxiliary network to learn the domain distinction. To augment informative features regarding the domain characteristic,
we treats the domain indicator directly as the ID feature input. The domain indicator is first mapped into embedding vectors and concatenated with other features. The auxiliary network then compute forward pass with respect to the concatenated features to gets it output. 
Denote the output  of star topology FCN  as $s_m$ and the output  of  auxiliary network as $s_a$. $s_m$ and $s_a$ are added to get the final logits. Then we apply softmax to the final logits and get the CTR prediction as:
\begin{equation}
    \textrm{softmax}(s_m+s_a). 
\end{equation}
As shown in Figure~\ref{fig:shadow}, the auxiliary network is much simpler than the main network, which is a two-layer fully connected neural network in our implementation. The simple architecture makes the domain features to directly influence to the final prediction.

Denote $\hat{y}^p_i$ the predicted probability for the i-th instance in the $p$-th domain and
% $\Theta_{sh}$  the parameters set of the shared parameter and $\Theta_{sp}$  the set of the domain-specific parameter. 
$y^p_i \in \{0,1\}$ the ground truth. We minimize the cross entropy loss function  between the $\hat{y}^p_i$ and label $y^p_i$ in all domains as:
\begin{align}
    \min-\sum_{p=1}^{M}\sum_{i=1}^{N_p} y^p_i\mathrm{log}(\hat{y}^p_i)-(1-y^p_i)\mathrm{log}(1-\hat{y}^p_i),
\end{align}.







